TRADE: Transducer-Augmented Decoder for Speech LLM

Speech Large Language Models (Speech LLMs) lack a principled mechanism for streaming inference: their label-synchronous generation has no acoustic-frame alignment, making real-time decoding and end-of-utterance detection difficult. We propose TRADE TRansducer-Augmented DEcoder, which augments a multimodal LLM with a transducer branch that shares the audio encoder and uses the LLM's hidden states directly as the prediction network -- coupling frame-synchronous acoustic alignment with the LLM's linguistic reasoning. Three design choices make the system accurate, streamable, and long-form capable: (1)Tightly coupled dual vocabularies -- a compact transducer vocabulary derived from the LLM vocabulary, enabling zero-cost score fusion; (2)Chunk-synchronized streaming training with gradient stopping, eliminating the train-inference mismatch at offline-equivalent memory cost; and (3)Localized Decoder Audio Attention (LDAA), a causal sliding window that caps KV-cache memory independently of utterance length. A single TRADE checkpoint supports offline and streaming decoding across a continuous range of latency operating points. TRADE achieves 6.71% average WER on the Open ASR Leaderboard, while the streaming recognition with 960ms chunk size reaches 8.40% from the same checkpoint. On long-form speech, it obtains 3.64% WER on TED-LIUM and 10.88% on Earnings-22 without external segmentation. TRADE provides sentence-end punctuation timestamps that, when combined with acoustic voice activity detection (VAD), improve end-of-utterance detection by +0.03 F_1 over acoustic VAD alone.

==> sections/broader_impacts.tex <==
% ===============================================================
\section{Broader Impacts}
\label{sec:broader_impacts}

Improved streaming ASR can benefit a wide range of accessibility and communication applications.
Real-time captioning for deaf and hard-of-hearing individuals, live transcription for telehealth consultations, and voice-driven interfaces for users with motor impairments are among the most direct beneficiaries of lower-latency, higher-accuracy speech recognition.
In healthcare settings, accurate ambient ASR reduces clinician documentation burden and can improve the fidelity of clinical records.

The same streaming capabilities that enable accessibility tools could also facilitate unauthorized audio surveillance or eavesdropping.
We note, however, that \DAT{} is not released as a public model or API, and the capabilities demonstrated in this paper do not substantially exceed those of already-public systems such as Whisper~\citep{radford2023robust}.
Any deployment of streaming ASR technology should be accompanied by appropriate consent frameworks, transparency to users whose speech is being transcribed, and compliance with applicable privacy regulations.

Regarding environmental impact, training \DAT{} on 153{,}000 hours of audio required significant compute (16$\times$H200 GPUs for 35{,}000 steps); researchers considering replication should weigh this cost and, where possible, reuse the released checkpoints when they become available.


==> sections/discussion.tex <==
% ===============================================================
\section{Discussion}
\label{sec:discussion}

\subsection{Extensions to Speech Understanding Tasks}

Beyond ASR, the \DAT{} architecture is well-positioned to extend to a range of speech understanding tasks. We discuss the most promising directions.

\paragraph{Speaker diarization.} Diarization — assigning each spoken segment to a speaker identity — is a natural fit for the frame-synchronous transducer. The joint network already operates at the level of individual encoder frames, making it straightforward to introduce a speaker-conditioned branch: speaker embeddings extracted from a separate encoder (e.g.\ x-vector or WavLM speaker head) can be injected into the joint network alongside the acoustic and LLM states. The transducer's blank/non-blank decision then serves a dual purpose — advancing the acoustic frame \emph{and} signalling speaker transitions. Multi-speaker ASR, where overlapping speech from distinct speakers is transcribed with speaker labels, follows as a direct extension. This is particularly compelling in the streaming setting, where the frame-synchronous read/write loop naturally interleaves transcription and speaker-change detection without requiring a separate diarization post-processing step.

\paragraph{Speech translation.} The LLM backbone is inherently multilingual and accustomed to sequence-to-sequence generation, making speech translation a low-friction extension. One approach treats translation as a second decoding target: a translation head shares the LLM's hidden states while the transducer continues to supervise frame alignment on the source language. Alternatively, the transducer vocabulary can be defined over target-language tokens directly, allowing the joint network to control frame consumption in the source while the LLM generates fluent target-language output. The chunk-based synchronised training scheme applies without modification, enabling streaming speech translation with the same latency guarantees as streaming ASR.

\paragraph{Spoken language understanding.} Tasks such as intent detection, slot filling, and named entity recognition over speech benefit from tight acoustic-semantic coupling. In \DAT{}, the LLM component naturally produces rich contextual representations at every token position, while the transducer's alignment constrains which acoustic frames contribute to each semantic unit. Fine-tuning the LLM with task-specific heads on top of the fused hidden states is a direct path to joint acoustic-semantic modelling, without needing a separate ASR-then-NLU pipeline. This has practical value for voice assistants and clinical documentation, where structured extraction must be performed in real time.

\paragraph{Spoken question answering.} Spoken QA requires simultaneously processing the acoustic content of a question and retrieving or generating a factual answer — a task that places high demand on both acoustic fidelity and linguistic reasoning. \DAT{} is naturally suited here: the transducer controls frame consumption to ensure no acoustic detail is missed, while the LLM's language prior drives answer generation. The fused decoding mechanism can be extended to condition on a retrieved context, enabling retrieval-augmented spoken QA. In the streaming setting, the chunk-based synchronisation scheme allows the system to begin generating an answer before the spoken question is complete, reducing response latency in dialogue scenarios.

\paragraph{End-of-utterance and turn-taking.} The transducer's frame-consumption mechanism provides a principled end-of-utterance (EOU) signal: decoding terminates when all $T$ encoder frames are consumed, with no reliance on EOS token generation or external voice activity detection. In multi-turn dialogue scenarios this directly governs response triggering and turn-taking latency. Extending \DAT{} to model conversational structure — distinguishing speaker turns, backchannels, and interruptions — is a further natural step enabled by the per-frame decision granularity of the transducer.

\paragraph{Long-form ASR.} Long-form transcription of meetings, lectures, and broadcast media is an increasingly important practical target. The Open ASR Leaderboard~\citep{srivastav2025openasr}, which benchmarks 86 systems across short- and long-form English tracks, finds that transducer- and CTC-based decoders achieve superior real-time factors compared to attention decoder models, making them better suited for long-form and batched processing despite often trailing on short-utterance WER. \DAT{} is naturally positioned for this regime: the Localized Decoder Audio Attention (Section~\ref{sec:windowed}) bounds the LLM's KV-cache to a fixed sliding window regardless of utterance length, preventing the quadratic memory growth that limits attention-only Speech LLMs on long inputs. The transducer's frame-synchronous alignment further avoids the repetition and hallucination artifacts common in encoder-decoder models on long audio. Extending the current short-form training and evaluation to long-form benchmarks, and validating the memory and latency advantages at scale, is a direct next step.

